Stochastic Amortization: A Unified Approach to Accelerate Feature and Data Attribution

Many tasks in explainable machine learning, such as data valuation and feature attribution, perform expensive computation for each data point and are intractable for large datasets. These methods require efficient approximations, and although amortizing the process by learning a network to directly predict the desired output is a promising solution, training such models with exact labels is often infeasible. We therefore explore training amortized models with noisy labels, and we find that this is inexpensive and surprisingly effective. Through theoretical analysis of the label noise and experiments with various models and datasets, we show that this approach tolerates high noise levels and significantly accelerates several feature attribution and data valuation methods, often yielding an order of magnitude speedup over existing approaches.

==> inserts/banzhaf_target_versus_prediction_external.tex <==
\begin{figure*}[ht]
\centering
\includegraphics[width=\linewidth]{images/banzhaf_target_versus_prediction_external.pdf}
\vspace{-0.22in}
\caption{Comparison of the estimation error between noisy labels and amortized predictions for Banzhaf value feature attributions (external data points). Noisy labels were generated using the MSR estimator with different numbers of samples. Top: using raw estimates as noisy training labels. Bottom: normalizing each noisy training label separately to have unit norm for each class.} \label{fig:banzhaf-target-versus-prediction-external}
\end{figure*}

==> inserts/lime_target_versus_prediction_external.tex <==
\begin{figure*}[ht]
\centering
\includegraphics[width=\linewidth]{images/lime_target_versus_prediction_external.pdf}
\vspace{-0.22in}
\caption{Comparison of the estimation error between noisy labels and amortized predictions for LIME feature attributions (external data points). Noisy labels were generated using LIME's least squares estimator with different numbers of samples. Top: using raw estimates as noisy training labels. Bottom: normalizing each noisy training label separately to have unit norm for each class.} \label{fig:lime-target-versus-prediction-external}
\end{figure*}

==> inserts/shapley_compute_trainsamples_logscale.tex <==
\begin{figure*}[ht!]
\centering
\includegraphics[width=0.27\linewidth, trim={0cm 0 26.7cm 0}, clip]{images/shapley_compute_trainsamples_logscale.pdf}
\vspace{-0.12in}
\caption{Estimation error for amortization and KernelSHAP with different dataset sizes given equivalent compute shown in log scale.} \label{fig:shapley-compute-trainsamples-logscale}
\end{figure*}
